Skill-based Model-based Reinforcement Learning

Model-based reinforcement learning (RL) is a sample-efficient way of learning complex behaviors by leveraging a learned single-step dynamics model to plan actions in imagination. However, planning every action for long-horizon tasks is not practical, akin to a human planning out every muscle movement. Instead, humans efficiently plan with high-level skills to solve complex tasks. From this intuition, we propose a Skill-based Model-based RL framework (SkiMo) that enables planning in the skill space using a skill dynamics model, which directly predicts the skill outcomes, rather than predicting all small details in the intermediate states, step by step. For accurate and efficient long-term planning, we jointly learn the skill dynamics model and a skill repertoire from prior experience. We then harness the learned skill dynamics model to accurately simulate and plan over long horizons in the skill space, which enables efficient downstream learning of long-horizon, sparse reward tasks. Experimental results in navigation and manipulation domains show that SkiMo extends the temporal horizon of model-based approaches and improves the sample efficiency for both model-based RL and skill-based RL. Code and videos are available at https://clvrai.com/skimo

==> table/results.tex <==
\begin{table}
  \caption{Evaluation results of reinforcement learning approaches. We measure the number of successful subtasks (1 for Maze, 4 for FrankaKitchen, and 4 for CALVIN). Each method is evaluated for 100 independent episodes and the result is averaged over 5 different random seeds.}
  \label{tab:results}
  \centering
  \begin{tabular}{lccccc}
    \toprule
    \multicolumn{3}{c}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Performance}}                   \\
    \cmidrule(r){1-3} \cmidrule(r){4-6} 
    Method              & Skill-based                       & Model-based   & 
    
    Maze & FrankaKitchen & CALVIN \\
    \midrule
    Dreamer~\citep{hafner2019dream}             & \color{BrickRed}{\XSolidBrush}    & \color{OliveGreen}{\Checkmark} & \\
    SPiRL~\citep{pertsch2020spirl}               & \color{OliveGreen}{\Checkmark}    & \color{BrickRed}{\XSolidBrush}              & & &     \\
    SPiRL\,+\,Dreamer   & \color{OliveGreen}{\Checkmark}    & \color{OliveGreen}{\Checkmark}                & & &      \\
    \midrule
    SkiMo\,+\,SAC       & \color{OliveGreen}{\Checkmark}    & \color{BrickRed}{\XSolidBrush}               & & &  \\
    SkiMo w/o joint training       & \color{OliveGreen}{\Checkmark}    & \color{OliveGreen}{\Checkmark}               & & &  \\
    SkiMo (Ours)        & \color{OliveGreen}{\Checkmark}    & \color{OliveGreen}{\Checkmark}               & & &  \\
    \bottomrule
  \end{tabular}
\end{table}
